Will It Still Be True Tomorrow? Multilingual Evergreen Question Classification to Improve Trustworthy QA

Large Language Models (LLMs) often hallucinate in question answering (QA) tasks. A key yet underexplored factor contributing to this is the temporality of questions -- whether they are evergreen (answers remain stable over time) or mutable (answers change). In this work, we introduce EverGreenQA, the first multilingual QA dataset with evergreen labels, supporting both evaluation and training. Using EverGreenQA, we benchmark 12 modern LLMs to assess whether they encode question temporality explicitly (via verbalized judgments) or implicitly (via uncertainty signals). We also train EG-E5, a lightweight multilingual classifier that achieves SoTA performance on this task. Finally, we demonstrate the practical utility of evergreen classification across three applications: improving self-knowledge estimation, filtering QA datasets, and explaining GPT-4o retrieval behavior.

==> Tables/RAGs_multihop.tex <==
\begin{table}[]
\begin{tabular}{l|l|l|ll}
HOTPOTQA & NoContext & Context &       &        \\ \hline
Dataset  & InAcc     & InAcc   & Delta & Amount \\
Full     & 0.360     & 0.744   & 0.383 & 20,000 \\
Ever     & 0.367     & 0.749   & 0.382 & 17,989 \\
Mutable  & 0.301     & 0.749   & 0.404 & 2,011  \\ \hline
MUSIQUE  & NoContext & Context &       &        \\ \hline
Dataset  & InAcc     & InAcc   & Delta & Amount \\
Full     & 0.107     & 0.285   & 0.178 & 20,000 \\
Ever     & 0.115     & 0.274   & 0.158 & 16,022 \\
Mutable  & 0.075     & 0.328   & 0.253 & 3,916 
\end{tabular}
\caption{Llama 3.1 multihop }
\label{tab:delta_rag}
\end{table}



==> Tables/RAGs_onehop.tex <==
\begin{table}[]
\begin{tabular}{l|l|l|ll}
NQ       & NoContext & Context &       &        \\ \hline
Dataset  & InAcc     & InAcc   & Delta & Amount \\
Full     & 0.389     & 0.772       & 0.383 & 20,000 \\
Ever     & 0.396     & 0.778       & 0.382 & 16,340 \\
Mutable  & 0.344     & 0.748       & 0.404 & 3,660  \\ \hline
TriviaQA & NoContext & Context &       &        \\ \hline
Dataset  & InAcc     & InAcc   & Delta & Amount \\
Full     & 0.656     & 0.834       & 0.178 & 20,000 \\
Ever     & 0.661     & 0.819       & 0.158 & 18,695 \\
Mutable  & 0.580     & 0.833       & 0.253 & 1,305 
\end{tabular}
\caption{Llama 3.1 one-hop}
\label{tab:my-table}
\end{table}

==> Tables/errors_examples.tex <==
% \begin{table}[]
% \footnotesize
% \begin{tabular}{lll}
% \hline
% Question                                                    & Dataset   & Predict   \\ \hline
% In what year did Leonardo DiCaprio \\ win an Oscar?            & Mutable   & Evergreen \\
% What is the lowest temperature \\ ever recorded in Antarctica? & Mutable   & Evergreen \\
% What is the length of the Amazon River?                     & Mutable   & Evergreen \\
% How many vitamins are there in total?                       & Mutable   & Evergreen \\ \hline
% What animal is depicted on the Porsche logo?                & Evergreen & Mutable   \\
% Which country is the largest?                               & Evergreen & Mutable   \\
% Which continent is located in all time zones?               & Evergreen & Mutable   \\
% What is the area of Liechtenstein?                          & Evergreen & Mutable   \\ \hline
% \end{tabular}
% \caption{EG-E5 model's errors in test part of dataset.}
% \label{tab:errors_models}
% \end{table}

% \begin{table}[]
% \footnotesize
% \begin{tabular}{lcc}
% \hline
% Question                                                    & Gold   & Predict   \\ \hline
% In what year did Leonardo \\ DiCaprio win an Oscar?            & Non-EG   & EG \\
% What is the lowest temperature \\ ever recorded in Antarctica? & Non-EG   & EG \\
% What is the length of \\ the Amazon River?                     & Non-EG   & EG \\
% How many vitamins are there in total?                       & Non-EG   & EG \\ \hline
% What animal is depicted on \\ the Porsche logo?                & EG & Non-EG   \\
% Which country is the largest?                               & EG & Non-EG    \\
% Which continent is located in \\ all time zones?               & EG & Non-EG    \\
% What is the area of Liechtenstein?                          & EG & Non-EG    \\ \hline
% \end{tabular}
% \caption{EG-E5 model's errors in test part of dataset.}
% \label{tab:errors_models}
% \end{table}

\begin{table}[]
\footnotesize
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
Question                                                    & Gold   & Predict   \\ \midrule
In what year did Leonardo \\ DiCaprio win an Oscar?            & Non-EG   & EG \\
What is the lowest temperature \\ ever recorded in Antarctica? & Non-EG   & EG \\
What is the length of \\ the Amazon River?                     & Non-EG   & EG \\
How many vitamins are there in total?                       & Non-EG   & EG \\ \midrule
What animal is depicted on \\ the Porsche logo?                & EG & Non-EG   \\
Which country is the largest?                               & EG & Non-EG    \\
Which continent is located in \\ all time zones?               & EG & Non-EG    \\
What is the area of Liechtenstein?                          & EG & Non-EG    \\ \bottomrule
\end{tabular}
}
\caption{EG-E5 model's errors in test part of dataset.}
\label{tab:errors_models}
\end{table}
